POET: Prompt Offset Tuning for Continual Human Action Adaptation

As extended reality (XR) is redefining how users interact with computing devices, research in human action recognition is gaining prominence. Typically, models deployed on immersive computing devices are static and limited to their default set of classes. The goal of our research is to provide users and developers with the capability to personalize their experience by adding new action classes to their device models continually. Importantly, a user should be able to add new classes in a low-shot and efficient manner, while this process should not require storing or replaying any of user's sensitive training data. We formalize this problem as privacy-aware few-shot continual action recognition. Towards this end, we propose POET: Prompt-Offset Tuning. While existing prompt tuning approaches have shown great promise for continual learning of image, text, and video modalities; they demand access to extensively pretrained transformers. Breaking away from this assumption, POET demonstrates the efficacy of prompt tuning a significantly lightweight backbone, pretrained exclusively on the base class data. We propose a novel spatio-temporal learnable prompt offset tuning approach, and are the first to apply such prompt tuning to Graph Neural Networks. We contribute two new benchmarks for our new problem setting in human action recognition: (i) NTU RGB+D dataset for activity recognition, and (ii) SHREC-2017 dataset for hand gesture recognition. We find that POET consistently outperforms comprehensive benchmarks. Source code at https://github.com/humansensinglab/POET-continual-action-recognition.

==> Sections/Method.tex <==
\newcommand{\task}[1]{{$\mathcal{US}^{(#1)}$}}
\newpage
\section{Preliminaries}
\label{sec_preliminaries}
% \begin{wrapfigure}{r}{0.35\textwidth} %this figure will be at the right
%     \centering
%     \includegraphics[width=0.35\textwidth]{Figures/Method_part1.pdf}
%     \caption{\textbf{Prompt Offset Tuning (POET)}: We propose to prompt offset the input feature embedding $x_e$ of the main model by learnable prompt parameters $P_{T}$ for privacy-aware few-shot continual action recognition. See Fig. \ref{fig: method, prompt selection} for prompt selection mechanism.}
%     % \vspace{-0.1in}
% \label{fig: method, main model}
% \end{wrapfigure}

%\subsection{Skeleton Action Recognition Using Graph Representations}
\noindent \textbf{Skeleton Action Recognition Using Graph Representations.}
Our input $x \in \mathbb{R}^{T \times J \times 3}$ is a video sequence of $T$ frames, each frame containing $J$ joints of the human body ($25$ joints) or hand skeleton ($22$ joints), with joint coordinates given in 3D Cartesian coordinate system. Such a skeleton action sequence is naturally represented as a graph topology $G = \{\mathcal{V}, \mathcal{E}\}$ with $\mathcal{V}$ vertices and $\mathcal{E}$ edges. Graphs are modeled using Graph Neural Networks (GNNs) \cite{dwivedi2022graph}, which can either be sparse graph convolutional networks (GCN) or fully connected graph transformers (GT). In Fig. \ref{fig: method, main model}, we define a GNN architecture as $f(x) = f_c \circ f_g \circ f_e(x)$; input $x$ is first passed through an input feature embedding layer $f_e$, followed by a graph feature extractor $f_g$ composed of a stack of convolutional layers (in GCNs) or attention layers (in GTs), and finally a classifier $f_c$ which predicts the action class label $y$. The input feature embedding is given by $x_e = f_e(x), x_e \in \mathbb{R}^{T \times J \times C_e}$.
% Typically, sparse GCNs have frame-wise graphs with spatial joints ($J$) as vertices in each graph. On the other hand, graph transformers model the entire spatio-temporal sequence of joints as a single fully connected graph with $T \times J$ vertices. (E.g. our CTR-GCN backbone for activity recognition benchmark)(Eg. our DG-STA backbone for hand gesture recognition benchmark)
%\vspace{-.5cm}
%\subsection{Problem Definition}

\begin{wrapfigure}[24]{r}{0.35\textwidth}
\vspace{-26pt}
\includegraphics[width=0.35\textwidth]{Figures/Method_part1.pdf}
\vspace{-8pt}
\caption{
\textbf{\footnotesize POET: \underline{P}rompt-\underline{o}ffs\underline{e}t \underline{T}uning} proposes to offset the input feature embedding $x_e$ of the main model by learnable prompt parameters $P_{T}$ for privacy-aware few-shot continual action recognition. 
We explain prompt selection mechanism in Fig. \ref{fig: method, prompt selection}.
% \textbf{POET: \underline{P}rompt-\underline{o}ffs\underline{e}t \underline{T}uning}: We propose to prompt offset the input feature embedding $x_e$ of the main model by learnable prompt parameters $P_{T}$ for privacy-aware few-shot continual action recognition. 
% See Fig. \ref{fig: method, prompt selection} for prompt selection mechanism.
}
\label{fig: method, main model}
% \vspace{-24pt}
\end{wrapfigure}
\noindent \textbf{Problem Definition.}
\label{method: problem def.}
Given a base trained model $\mathcal{M}$ deployed on a user's device, we would like to learn a new set of classes in $T$ subsequent user sessions 
%Few-Shot Class Incremental Action Recognition is a continual learning paradigm where a model deployed on a user's device sequentially adapts to learn a series of $T$ user sessions 
(also called tasks) \{$\mathcal{US}^{(1)},..., \mathcal{US}^{(T)}$\} corresponding to training datasets \{$\mathcal{D}^{(1)},..., \mathcal{D}^{(T)}$\}; where $\mathcal{D}^{(t)} = {(x_i^t, y_i^t)}_{i=1}^{\mid \mathcal{D}^{(t)} \mid}$ are skeleton action sequence and label pairs provided by the user, $x_i^t \in \mathbb{R}^{T \times J \times 3}$, $y_i^t \in \mathbb{R}^{\mathcal{Y}^{(t)}}$. In each session, the user typically provides a few training instances $F$ (e.g. $F \leq 5$) for each of the $N$ new classes being added, such that $|\mathcal{D}^{(t)}| = NF$. The base model's session $\mathcal{UB}^{(0)}$ is assumed to have a large number of default action classes $\mathcal{Y}^{(0)}$ trained on sufficient data $\mathcal{D}^{(0)}$, which is most often proprietary and cannot be accessed in later user sessions. In each session, the user adds new action classes, i.e. $\mathcal{Y}^{(t)} \cap \mathcal{Y}^{(t')} = \emptyset, \forall t \neq t'$\footnote{\scriptsize We make this assumption considering this is a first of such efforts; allowing for overlapping action classes and users to `update' older classes would be interesting extensions of our proposed work.}. Due to the aforementioned privacy constraints, in any training session $\mathcal{US}^{(t)}$, the model has access to only $\mathcal{D}^{(t)}$; after training, this data is made inaccessible for use in subsequent sessions (no exemplar or prototypes stored). After training on every new session $\mathcal{US}^{(t)}$, the model is evaluated on the test set of all classes seen so far $\cup_{i=0}^t \mathcal{Y}^{(i)}$. The challenge is to alleviate forgetting of old classes while not overfitting to the user-provided samples. One could view our setting as privacy-aware few-shot class-incremental learning for human actions, a problem of practical relevance -- especially in human action recognition -- which has not received adequate attention yet, to the best of our knowledge.

%and is referred to as a N-way F-shot session. For e.g., learning 5 novel classes in each new task using 5 user samples is a 5-way 5-shot user session. 

 
% \vspace{-.5cm}

\section{Methodology: POET}
\textbf{Overview:}
In Sec \ref{method: construct prompt}, we first define our spatio-temporal prompt offsets (called POET) to prompt tune a GNN (see Fig. \ref{fig: method, main model}), explaining why it is different from prompt tuning transformers for text, images and videos. Next, in Sec. \ref{method: selection} we explain our novel end-to-end optimization of the prompt codebook which enables prompt selection across novel continual tasks even though our query function is pretrained only on base task data (Fig. \ref{fig: method, prompt selection}). Finally, our proposed prompt attachment \textit{adds} the same number of prompts as the number of temporal frames in the input, such that the \textit{selected prompts are temporally consistent with the input} (Sec \ref{method: ordering}).   

\subsection{Constructing Spatio-Temporal Prompt Offsets}
\label{method: construct prompt}
Learnable (or soft \cite{lester2021power}) prompts are parameter vectors in a continuous space which are optimized to adapt the pretrained frozen backbone model to each continual task. We define our spatio-temporal prompt offsets $P_{T'}$ as a set of $T'$ prompts, each prompt $P_i$ having length equal to the \#joints in a frame $J$ and feature dimension same as the input feature embedding $x_e$, i.e., $P_{i} \in \mathcal{R}^{J \times C_e}$.

\noindent \textbf{Prompt tuning of GNNs?}
There exist prior works which generalize transformers to graphs \cite{dwivedi2020generalization, mialon2021graphit, chen2019construct}. \textit{Then why is it non-trivial to attach prompts to a GNN?} NLP transformers \cite{vaswani2017attention} treat sentences as a fully connected graph with every word attending to every other word in the sentence as there are no explicit word interactions or edge information in sentences \cite{dwivedi2022graph}. It is the same case with vision transformers \cite{dosovitskiy2020image} which compute attention among all image patches. This lack of pre-defined edge information makes it straightforward to prepend an arbitrary number of tokens for the MHSA mechanism.
% is invariant of the number of tokens. 
However, our spatio-temporal input is a natural graph skeleton of the human joint-bone structure and \textit{has a well defined edge connectivity}. This edge information is exploited as inductive bias in GNNs. If we treat joints as tokens and concatenate prompts along spatial or temporal dimensions, not only does the graph topology lose semantic meaning, but the forward pass operation becomes undefined (especially in GCNs). Hence, we denote our unknown prompt attachment function as $f_p$. The logit distribution can then be obtained as:

\begin{equation} \label{eqn: 1}
    y = f(x, P_{T'}) = \textcolor{RedOrange}{f_c} \circ \textcolor{cyan}{f_g} \circ f_p(\textcolor{cyan}{f_e}(x), \textcolor{RedOrange}{P_{T'}}). 
\end{equation}

% \begin{equation} \label{eqn: 1}
%     f_p(x_e, P_{T'}) = x_e' , \qquad x_e' \in \mathcal{R}^{T \times J \times C_e}.
% \end{equation}

\noindent In every subsequent session $t > 0$, the classifier output dimension expands by $N$ to accommodate for the new classes. Importantly, disparate from most existing continual prompt tuning works, our feature extractor backbone $f_g$ is trained \textit{only on the base class data $\mathcal{D}^{(0)}$} and will never itself be fine-tuned on action semantics from any of the continual sessions $\mathcal{US}^{(t)}, t>0$. After the base session training, parameters of \textcolor{cyan}{$f_g, f_e$} are frozen, and only the prompt-associated parameters and classifier \textcolor{RedOrange}{$f_c$} are updated, refer to Fig. \ref{fig: method, main model}.

\subsection{Prompt Selection and Attachment Mechanism}
\label{method: selection}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{Figures/Method_part2.pdf}
\vspace{-0.1in}
\caption{\textbf{Construction of our prompts $P_{T}$}: Input-dependent query $Q$ is matched with keys $\boldsymbol{K}$ using \textit{sorted} cosine similarity to get an ordered index sequence $(s_i)_{i=1}^{T}$ of the top $T$ keys. This ordered index sequence is used to select the corresponding ordered prompt sequence $P_{T}$ from prompt pool $\boldsymbol{P}$. We \textit{add} $P_T$ to $x_e$ from main model (Fig. \ref{fig: method, main model}), thereby offsetting it. Our experimental evaluation confirms that such an additive 
spatio-temporal prompt offsetting can balance the plasticity to learn new classes from few-shot gestures, while maintaining the stability on the previously learned classes.
% Additive spatio-temporal prompt offsets are all we need for continually learning new user actions!
}
\label{fig: method, prompt selection}
\end{figure*}

\subsubsection{Prompt Codebook Design.} 
As mentioned in Sec.~\ref{sec: continual prompt tuning}, to encourage knowledge sharing in our few-shot continual setting, we choose to construct a single prompt pool $\boldsymbol{P}$, sharing encoded knowledge across all tasks:

\begin{equation} \label{eqn: 2}
    \boldsymbol{P} = \{P_1,.. P_i, ..., P_M \}, \qquad P_{i} \in \mathcal{R}^{J \times C_e} ; M = \textrm{\#prompts at time t}.
\end{equation}

\noindent For the prompt selection process (Fig. \ref{fig: method, prompt selection}), we construct a bijective key-value codebook, treating prompts in the pool $\boldsymbol{P}$ as values and defining learnable key vectors as $\boldsymbol{K} = \{K_1,.., K_i,.., K_M \}, K_i \in \mathcal{R}^{C_e}$. A query $Q$ and keys $\boldsymbol{K}$ matching process is used to find and fetch the $T'$ closest values (prompts in the pool). This vector quantization process is enabled by a query function $f_q(x)$. The query function is an encoder which maps an input instance $x$ to a query $Q$ as:

\begin{equation} \label{eqn: 3}
    Q = f_q(x) = \textcolor{RedOrange}{f_{QA}} \circ \textcolor{cyan}{f_g'} \circ \textcolor{cyan}{f_e'} (x), \qquad x \in \mathbb{R}^{T \times J \times 3} \rightarrow Q \in \mathcal{R}^{C_e}.
\end{equation}

\noindent where the \textit{query adaptor} \textcolor{RedOrange}{$f_{QA}$} is a fully connected layer mapping the \textcolor{cyan}{$f_g'$} output dimension to the desired prompt embedding dimension $C_e$. The most relevant $T'$ prompt indices are then selected using cosine similarity $ \gamma(.)$ as: 

\begin{equation} \label{eqn: 4}
 \argmax_{T'} \gamma (f_q(x), \boldsymbol{K}).
\end{equation}

\noindent \textbf{Coupled Optimization in incremental steps, $t>0$.} 
To move queries closer to their aligned $T'$ keys during training, we use a vector quantization clustering loss inspired from VQ-VAE \cite{van2017neural} and similar to Learning to Prompt (L2P) \cite{wang2022learning}:

\begin{equation} \label{eqn: 5}
 \max_{\theta_{QA}, \theta_{K_{T'}}} \lambda \Sigma_{i=1}^{T'} \gamma (f_q(x), K_i).
\end{equation}

\noindent Even though L2P \cite{wang2022learning} and Dual-P \cite{wang2022dualprompt} serve as strong starting points for our continual prompt selection mechanism, they decouple the optimization of prompt pool from the keys. This implies that the cross entropy loss for every new task ($t>0$) only updates the classifier and prompts, but not the keys and query function, as the $\argmax$ operator in Eq. \ref{eqn: 5} 
% generates a non-smooth binary mask of selected key indices 
prevents backpropagation of gradients to the keys. \textit{However, this would be a fatal flaw in our setting:} We assume no large-scale pretraining on a superset of semantic knowledge the model could potentially see during its lifetime. Thus, for all practical purposes, our query function $f_q$ is pretrained \textit{only on the base class data $\mathcal{D}^{(0)}$}. For it to discern all old and new class samples, it must be updated as the model learns new classes. As shown in Fig \ref{fig: method, prompt selection}, we propose to couple this optimization process such that the cross entropy loss for new tasks updates (i) the classifier \textcolor{RedOrange}{$f_c$}, (ii) selected prompts \textcolor{RedOrange}{$P_{T'}$}, (iii) keys \textcolor{RedOrange}{$K_{T'}$}, as well as (iv) query adaptor \textcolor{RedOrange}{$f_{QA}$}. We freeze the query feature extractor layers \textcolor{cyan}{$f_g', f_e'$} in $t>0$ to prevent catastrophic forgetting of base knowledge. We approximate the gradient by the straight-through estimator reparameterization trick as in \cite{van2017neural, bengio2013estimating}. Our proposed coupled cross entropy loss:

\begin{equation} \label{eqn: 6}
    \min_{\theta_{QA}, \theta_{K_{T'}}, \theta_{P_{T'}}, \theta_{f_c}} \mathcal{L}(f(x, P_{T'}), y).
\end{equation}

\noindent This coupled mechanism establishes a \textit{prompt optimization framework which is imperative to prompt tuning without pretraining}. It enabled us to design our spatio-temporal prompt offsets described next.
% in Sections \ref{method: attachment} and \ref{method: ordering}. 

\noindent \textbf{Additive Prompt Attachment.} We achieve best results when the number of selected prompts $T'$ in $P_{T'}$ is same as the number of temporal frames in the input skeleton, $T$. We find a naive addition operation yields best results empirically: 
\begin{equation} \label{eqn: 7}
 f_p(x_e, P_{T'}) = x_e + P_{T'}, T' = T.
\end{equation}

\noindent Note, we use $T$ instead of $T'$ in the following sections, and in Figures \ref{fig: method, main model} and \ref{fig: method, prompt selection}.

\subsection{Ordered Prompt Sequence Selection}
\label{method: ordering}
Since the number of selected prompts corresponds with the number of temporal frames in the input skeleton sequence, we make the prompt selection mechanism temporally consistent with respect to the input. We achieve this by simply sorting the top $T$ keys based on their the query-key cosine similarity to get an \textit{ordered key index sequence $(s_i)_{i=1}^{T}$}, replacing a naive top $T'$ index selection in Eq. \ref{eqn: 5} as: 

\begin{equation} \label{eqn: 8}
 \argsort_{(s_i)_{i=1}^{T} \subseteq [1, M]} \gamma (f_q(x), \boldsymbol{K}).
\end{equation}

\noindent We use this order $(s_i)_{i=1}^{T}$ to read the prompt pool memory and select final prompts $P_T$.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{Figures/ordering_matrices.pdf}
\vspace{-0.1in}
\caption{\textbf{Task-level Prompt Sequence Analysis.} Here we visualize the order $(s_i)_{i=1}^{T}$ in which the $M = 64$ prompts in the prompt pool are selected at train time, with the addition of 5 new classes in each user session $\mathcal{US}^{(t)}$. X-axis: prompt index number, Y-axis: index position in selected sequence. % Bottom left of each plot, we have the test accuracy only for the 5 `New' classes learnt in that task. 
\textit{Bottom:} Even though the same 64 prompts are selected and updated, the ordered prompt selection helps POET learn new knowledge better and renders temporal consistency. \textit{Top:} The no sorting case uses the default sequence (hence diagonal matrices), giving equal importance to all prompts.}
\label{fig: ordering_qual_vis}
\end{figure*}
\vspace{-0.2in}

\begin{figure*}[bh]
\centering
\includegraphics[width=0.99\textwidth]{Figures/pool_collapse.pdf}
\vspace{-0.1in}
\caption{\textbf{$M>T$ Case:} \textit{Prompt Pool Collapse.} Certain prompt indices remain completely unused across all tasks. \textit{Our POET pool expansion} algorithm alleviates pool collapse.}
\label{fig: pool collapse}
\end{figure*}

\subsection{Mitigating Prompt Pool Collapse}
After coupling the prompt pool and keys, we observed in our initial experiments with pool size $M > T$ that the same set of prompts are getting selected across training iterations and incremental steps (Figure \ref{fig: pool collapse}, A). More concretely, 
% at the start of base session $\mathcal{US}^{(0)}$, a random set of key indices and corresponding prompts is selected and optimized. 
as the vector quantization loss (Equation \ref{eqn: 6}) brings the query close to the selected keys, the same set of active prompts get selected and optimized in each iteration, not using the other prompts at all. This is similar to the well known issue of ``codebook collapse" in VQ-VAE \cite{williams2020hierarchical, dhariwal2020jukebox, zheng2023online}. Based on this observation, we design two prompt pool update mechanisms for the 2 cases: 
\begin{enumerate}
    \item $M = T, \forall t$. \textbf{No pool expansion, Algorithm \ref{alg:POET}}. All the prompts are selected in all tasks. But, the \textit{order of their selection $(s_i)_{i=1}^{T}$} varies with each input instance and is discriminative such that certain prompts tend to appear before others in $(s_i)_{i=1}^{T}$ for different input semantics. In Figure \ref{fig: ordering_qual_vis}, we visualize the position occupied by prompt indices in the ordered sequence $(s_i)_{i=1}^{T}$. Entropy increase across tasks $t=1$ to $t=4$ shows that our selection mechanism learns to select a unique temporal code for all inputs. 
    \item $M = T + (R * t), t > 0$. \textbf{Expand pool with R prompts}. We also propose an order-aware prompt pool expansion algorithm (supplementary) that selects prompts from an expanded pool in a temporally coherent manner, for $t>0$. This alleviates prompt pool collapse as shown in Figure \ref{fig: pool collapse}, B.  
\end{enumerate}


\vspace{0.0cm}
\begin{algorithm*}[h]
% \scriptsize
\footnotesize
\vspace{-2pt}
\caption{\small POET (No pool expansion case) at Train Time, $t \geq 1$}\label{alg:POET}
\begin{algorithmic}
\State \textbf{Input:} Query function $f_q$, prompt keys $\boldsymbol{K}=\{K_j\}_{j=1}^M$, prompt pool $\boldsymbol{P}=\{P_j\}_{j=1}^M$; main model input embedding layer $f_e$, graph feature extractor $f_g$, classifier $f_c$ pretrained from time $t-1$. \textbf{Note, M=T}
\State \textbf{Initialize:} $\boldsymbol{P}, \boldsymbol{K}$ from $t-1$; Expand $f_c$ by $N$ new classes. Initialize $f_c$ as: (i) copy $f_c^{old}$ weights, (ii) $f_c^{new} \leftarrow Mean(f_c^{old})$ 
\State \textbf{Freeze:} query layers \textcolor{cyan}{$f_g', f_e'$}; main model layers \textcolor{cyan}{$f_e, f_g$}
\State \textbf{for} epochs and batch ${(x_i^t, y_i^t)}_{i=1}^{NK}$ do
    \State \hskip0.8em 1. Compute query feature $Q = f_q(x)$
    \State \hskip0.8em 2. Compute cosine similarity $\gamma(.)$ b/w query $Q$ and keys $\boldsymbol{K}$
    \State \hskip0.8em 3. \textcolor{black}{Sort} $\gamma(.)$; Get \textcolor{black}{ordered key index sequence} $K_{T} = (s_i)_{i=1}^{T}$ (Equation \ref{eqn: 8})
    \State \hskip0.8em 4. Index prompt pool $\boldsymbol{P}$ in order $(s_i)_{i=1}^{T}$ $\rightarrow$ Get final prompt $P_{T}$
    \State \hskip0.8em 5. Compute input embedding $x_e = f_e(x)$
    \State \hskip0.8em 6. Attach/\textbf{Add} prompt as per Equation \ref{eqn: 7}, use prompted input to get prediction.
    \State \hskip0.8em 7. Use clustering loss (Equation \ref{eqn: 5}) to \textbf{update} query adaptor $QA$, keys $K_{T}$ 
    \State \hskip0.8em 8. Use cross entropy loss (Equation \ref{eqn: 6}) to \textbf{update} $QA, K_{T}, P_{T}, f_c$
    \State \hskip0.8em 9. \textbf{Classifier $f_c$} is (i) cosine classifier for NTU RGB+D; \\  \hskip1.6em (ii) regular FC layer, but freeze $f_c^{old}$ by zeroed gradients for SHREC 2017,
    % \State \hskip0.6em \textbf{end}
\State \textbf{end} \textcolor{orange}{// See $t=0$ training protocol in Supplementary Algorithm 2.} 
\vspace{-2pt}
\end{algorithmic}
\end{algorithm*}

\section{Discussion}
\subsection{Differences From Existing Continual Prompt Tuning Works}
\begin{enumerate}
    \item \textbf{Enable prompt tuning w/o extensive pretraining} As explained in Section \ref{method: selection}, we optimize prompts, keys, and query adaptor in an end-to-end coupled optimization in order to update the query on unseen classes. Before us, CODA-P \cite{smith2023coda} also coupled their keys with the prompt pool. However, their coupling was done by using the cosine similarity to weigh all prompts in the pool, forming a `soft prompt selection' instead of our `ordered hard prompt selection'. Most importantly, these methods use a well pretrained query function which does not require updates. Finally, due to our lightweight backbone, there is significant forgetting from the classifier and we follow Algorithm \ref{alg:POET} line 9 to mitigate the same.    
    \item \textbf{Spatio-temporal prompt offsets for GNNs:} Before us, PIVOT \cite{villa2023pivot} trains separate spatial and temporal prompts on a pretrained CLIP for video continual learning. However, our \textbf{additive} spatio-temporal prompt offsets are a \textit{simple plug-and-play for prompt tuning of any GNN architecture}, making it invariant to datasets, backbones and input sizes. POET is also a \textit{prompt-only strategy} that does not require additional replay or regularization for continual learning. 
\end{enumerate}

\subsection{Interpreting Prompt Offset Tuning of GNNs}
Even though our inspiration for POET came from existing continual prompt tuning works \cite{wang2022learning, wang2022dualprompt, smith2023coda, bowman2023carte}, our additive prompt offsets are open to interpretation. (i) Adding our selected prompts $P_T$ to input feature embedding $x_e$ acts like an input-dependent transformation for spatio-temporal joints. (ii) As our prompts have same size as $x_e$, it can also be thought of as a learned prompt encoding, bearing similarity with learnable position encoding works \cite{liu2020learning, li2021learnable, dwivedi2022graph}. Our work is different as the purpose of prompt offsets is to dynamically condition the input for adapting the backbone continually, instead of learning positions. (iii) Finally, it also bears similarity with auto-decoders like DeepSDF \cite{park2019deepsdf} which learn latent codes for each data point (or style, shape) and use relevant codes along with a frozen decoder at inference.  



==> Sections/X_tables.tex <==
\newcommand{\task}[1]{{$\mathcal{T}^{(#1)}$}}
\begin{table*}[ht]
% \scriptsize
% \footnotesize
\setlength{\tabcolsep}{3pt}
\vspace{-0.2in}
\centering
\caption{\textbf{Prompt Selection Mechanism Analysis:} POET on NTU RGB+D dataset. `w/o' denotes removing that component from our method POET. `Avg' accuracy metric is biased towards `Old' classes accuracy, $A_{HM}$ is a good indicator of trade-off between `New' and `Old'. All metrics $\uparrow$.}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lllllllllllllll@{}}\toprule 
& \task{0} 
& \multicolumn{3}{c}{\task{1}} 
& \multicolumn{3}{c}{\task{2}} 
& \multicolumn{3}{c}{\task{3}} 
& \multicolumn{4}{c}{\task{4}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}  \cmidrule(l){12-15} 
Method & Base  & Old & New & Avg & Old & New & Avg & Old & New & Avg & Old & New & \textbf{Avg} & $\boldsymbol A_{HM}$  \\
\hline
w/o prompts (FE) & 88.4 & 76.5 & 59.1 & 74.5 & 67.9 & 51.4 & 66.3 & 50.4 & 40.8 & 49.5 & \cellcolor{gray!20}39.2 & \cellcolor{gray!20}46.8 & \cellcolor{gray!20}39.9 & 42.7 \\
w/o coupled optim. & 88.0 & 85.3 & 61.6 & 82.8 & 78.0 & 50.6 & 75.3 & 67.1 & 55.1 & 65.8 & 56.5 & 51.3 & 56.1 & 53.8 \\
w/o clustering loss & 85.5 & 86.6 & 41.5 & 81.6 & 78.9 & 36.8 & 74.3 & 69.2 & 28.9 & 64.5 & 62.0 & 18.2 & 57.0 & 28.1 \\
w/o QA update & 87.9 & 84.7 & 66.3 & 82.8 & 80.9 & 45.5 & 77.4 & 70.1 & 59.5 & 69.1 & 59.4 & 52.8 & 58.7 & 55.9 \\
% old results:
% w/o Pool Expansion & 87.9 & 84.7 & 66.6 & 82.6 & 80.5 & 45.3 & 77.0 & 69.9 & 58.3 & 68.9 & \textbf{60.1} & 52.8 & \textbf{59.5} & 56.2 \\
% w/o Freeze Old Prompts & 87.9 & 84.8 & 67.1 & 82.9 & 80.8 & 44.9 & 77.3 & 70.1 & 59.5 & 69.1 & 59.5 & 54.6 & 58.6 & 56.9 \\
% Attach new prompts before & 87.9 & 84.8 & 66.6 & 82.7 & 80.7 & 45.8 & 77.2 & 70.2 & 59.2 &  68.9 & 59.3 & 54.1 & 58.8 & 56.6 \\
% \hline
% POET (Ours) & 87.9 & 84.7 & 66.0 & 82.6 & 80.1 & 45.8 & 77.0 & 69.9 & 59.2 & 68.8 &  \cellcolor{gray!20}59.3 & \cellcolor{gray!20}\textbf{57.4} & \cellcolor{gray!20}59.4 & \textbf{58.4} \\
w/o sorting & 88.2 & 84.5 & 63.6 & 82.2 & 78.5 & 45.2 & 75.2 & 70.0 & 56.2 & 68.8 & 59.9 & \cellcolor{gray!20}46.6 & 58.8 & 52.4 \\
\hline
POET ($M>T$) & 87.9 & 84.7 & 66.4 & 82.7 & 80.8 & 45.2 & 77.2 & 69.8 & 58.9 & 68.8 & 60.3 & 54.4 & 59.8 & 57.2 \\
POET ($M=T$) & 87.9 & 84.9 & 65.6 & 82.8 & 80.3 & 45.8 & 76.8 & 69.5 & 60.0 & 68.6 & \cellcolor{gray!20}59.3 & \cellcolor{gray!20}\textbf{57.4} & \cellcolor{gray!20}59.2 & \textbf{58.3} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{main ablation}
\end{table*}


\begin{table*}[t]
% \scriptsize
% \footnotesize
\setlength{\tabcolsep}{4pt}
% \vspace{-0.2in}
\centering
\caption{\textbf{Prompt Attachment Analysis:} Exploring prompt function $f_p$ and optimal number of prompts (NTU RGB+D dataset).}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lllllllllllllll@{}} \toprule 
& \task{0} 
& \multicolumn{3}{c}{\task{1}} 
& \multicolumn{3}{c}{\task{2}} 
& \multicolumn{3}{c}{\task{3}} 
& \multicolumn{4}{c}{\task{4}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}  \cmidrule(l){12-15} 
Method & Base & Old & New & Avg & Old & New & Avg & Old & New & Avg & Old & New & \textbf{Avg} & $\boldsymbol A_{HM}$  \\
\hline
CONC. temp, $T'=64$  & 88.6 & 69.7 & 75.6 & 70.3 & 62.5 & 60.2 & 62.4 & 48.7 & 60.0 & 49.8 & 33.6 & 50.5 & 35.1 & 40.3 \\
CONC. feat, $T'=64$  & 87.7 & 85.4 & 58.4 & 82.4 & 79.2 & 41.8 & 75.5 & 68.2 & 54.2 & 66.9 & 57.1 & 41.5 & 56.0 & 48.1 \\
\hline
ADD, $T'=1$ & 88.7 & 73.4 & 72.8 & 73.3 & 62.0 & 69.3 & 62.7 & 45.0 & 50.6 & 45.5 & 33.7 & 47.0 & 34.8 & 39.3 \\
\hline
ADD, $T'=64$ (Ours) & 87.9 & 84.9 & 65.6 & 82.8 & 80.3 & 45.8 & 76.8 & 69.5 & 60.0 & 68.6 & \cellcolor{gray!20}59.3 & \cellcolor{gray!20}57.4 & \cellcolor{gray!20}\textbf{59.2} & \textbf{58.3} \\
% Cross Attention & 88.1 & 2.5 & 0.0 & 2.2 & 0.0 & 20.1 & 2.0 & 0.0 & 20.0 & 1.8 & 0.0 & 19.8 & 1.65 & 0.0 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{prompt attachment}
\end{table*} 

\begin{table*}[t]
% \scriptsize
\setlength{\tabcolsep}{4pt}
\centering
\caption{Performance on NTU RGB+D~\cite{shahroudy2016ntu} \textbf{Activity Recognition benchmark}, based on CTR-GCN \cite{chen2021channel} backbone. Numbers indicate Test Accuracy (\%, $\uparrow$). After training on each incremental task, we report (i) performance of all old classes averaged (`Old'), (ii) only new classes (`New'), and (iii) Average of all classes seen so far (`Avg') to understand stability-plasticity trade-offs. We also report $A_{HM}$ in the last task. \textbf{Notation:} \textbf{\^} denotes standalone models trained and deployed for each task $T_i$ individually (note `Avg' is NA for these and `Old' refers to only base session \% for these); \textbf{$\dagger$} refers to storage and replay of all incremental session training data; \textbf{*} refers to concatenation of prompts along temporal dimension of input embedding $x_e$; and \textbf{**} concatenates along a rolled-out spatio-temporal dimension of $x_e$.}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lllllllllllllll@{}} \toprule 
& \task{0} 
& \multicolumn{3}{c}{\task{1}} 
& \multicolumn{3}{c}{\task{2}} 
& \multicolumn{3}{c}{\task{3}} 
& \multicolumn{4}{c}{\task{4}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}  \cmidrule(l){12-15} 
Method & Base & Old & New & Avg & Old & New & Avg & Old & New & Avg & Old & New & \textbf{Avg} & $\boldsymbol A_{HM}$  \\
\hline
Joint (Oracle)  & 88.4 &  &  & 79.0 &  &  & 71.0 &  &  & 66.8 &  &  & \cellcolor{gray!20}\textbf{63.5} &  \\
Joint POET &  & \multicolumn{3}{l}{} &  &  &  &  &  &  &  &  & \cellcolor{gray!20}\textcolor{red}{\textbf{67.2}} &  \\
% Task-Specific\^ &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
FE & 88.4 & 76.5 & 59.1 & 74.5 & 67.9 & 51.4 & 66.3 & 50.4 & 40.8 & 49.5 & \cellcolor{magenta!20}39.2 & \cellcolor{yellow!30}46.8 & 39.9 & 42.7 \\
FE, TS\^ & 88.4 & \cellcolor{magenta!20}76.5 & \cellcolor{yellow!30}59.1 & 74.5 & \cellcolor{magenta!20}77.8 & \cellcolor{yellow!30}39.4 & NA & \cellcolor{magenta!20}76.0 & \cellcolor{yellow!30}45.5 & NA & \cellcolor{magenta!20}72.1 & \cellcolor{yellow!30}38.8 & NA & NA \\
FE, frozen & 88.4 & 81.7 & 49.2 & 78.1 & 64.7 & 40.0 & 62.3 & 43.2 & 27.6 & 41.7 & \cellcolor{magenta!20}29.5 & \cellcolor{yellow!30}25.5 & 29.2 & 27.4 \\
FE, replay$\dagger$ & 88.4 & 73.5 & 70.1 & 73.1 & 59.2 & 71.0 & 60.4 & 61.8 & 59.4 & 61.6 & 60.3 & 28.8 & 57.7 & 39.0 \\
FT & 88.4 & \phantom{0}0.4 & 58.2 & \phantom{0}6.8 & \phantom{0}0.0 & 59.2 & \phantom{0}6.0 & \phantom{0}0.0 & 41.6 & \phantom{0}3.8 & \cellcolor{magenta!20}\phantom{0}0.0 & \cellcolor{yellow!30}25.1 & \phantom{0}2.1 & \phantom{0}0.0 \\
\hline
LWF \cite{li2017learning} & 88.4 & \phantom{0}0.5 & 74.0 & \phantom{0}8.7 & \phantom{0}0.0 & 31.5 & \phantom{0}3.2 & \phantom{0}0.0 & 31.4 & \phantom{0}2.9 & \phantom{0}0.0 & 23.1 & \phantom{0}1.9 & \phantom{0}0.0 \\
EWC \cite{kirkpatrick2017overcoming} & 88.4 & \phantom{0}0.0 & 57.4 & \phantom{0}6.4 & \phantom{0}0.0 & 62.2 & \phantom{0}6.2 & \phantom{0}0.0 & 33.9 & \phantom{0}3.1 & \phantom{0}0.0 & 28.9 & \phantom{0}2.4 & \phantom{0}0.0 \\
ER $\dagger$ & 88.4 & \phantom{0}0.4 & 59.8 & \phantom{0}7.0 & \phantom{0}6.1 & \phantom{0}5.2 & \phantom{0}6.0 & \phantom{0}6.8 & 42.2 & 10.0 & 10.1 & 32.2 & 12.0 & 15.4 \\
LUCIR \cite{hou2019learning} & 87.9 & \phantom{0}0.0 & 19.9 & \phantom{0}2.2 & \phantom{0}0.0 & 20.1 & \phantom{0}2.0 & \phantom{0}0.0 & 29.2 & \phantom{0}2.7 & \phantom{0}1.3 & \phantom{0}2.5 & \phantom{0}1.4 & \phantom{0}0.0 \\
 % &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
CODA-P \cite{smith2023coda}* & 87.4 & 86.1 & \phantom{0}4.0 & 76.3 & 76.0 & \phantom{0}0.3 & 68.4 & 65.9 & \phantom{0}0.2 & 59.7 & \cellcolor{magenta!20}60.9 & \cellcolor{yellow!30}\phantom{0}0.7 & \cellcolor{gray!20}55.7 & \phantom{0}1.3 \\
CODA-P \cite{smith2023coda}** & 87.6 & \phantom{0}4.9 & \phantom{0}7.4 & \phantom{0}4.5 & 31.7 & \phantom{0}0.0 & 28.8 & \phantom{0}0.5 & \phantom{0}1.6 & \phantom{0}0.6 & 35.4 & \phantom{0}0.7 & 31.1 & \phantom{0}1.3 \\
L2P \cite{wang2022learning}* & 88.6 & 88.4 & \phantom{0}0.0 & 78.5  & 78.5 & \phantom{0}0.0 & 70.7 & 70.1 & \phantom{0}0.0 & 63.7 & \cellcolor{magenta!20}\textbf{61.2} & \cellcolor{yellow!30}\phantom{0}0.0 & \cellcolor{gray!20}56.2 & \phantom{0}0.0 \\
L2P \cite{wang2022learning}**  & 84.7 & \phantom{0}3.0 & \phantom{0}0.4 & \phantom{0}2.7 & \phantom{0}3.1 & \phantom{0}0.0 & \phantom{0}2.8 & \phantom{0}2.8 & \phantom{0}0.0 & \phantom{0}2.6 & \phantom{0}2.4 & \phantom{0}0.4 & \phantom{0}2.2 & \phantom{0}0.6 \\
APT \cite{bowman2023carte}\^ & 86.6 & \phantom{0}NA & 29.2 & \phantom{0}NA & \phantom{0}NA & 30.6 & \phantom{0}NA & \phantom{0}NA & 35.9 & \phantom{0}NA & \phantom{0}NA & 35.0 & \phantom{0}NA & \phantom{0}NA \\
% ALICE \cite{peng2022few} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% NC-FSCIL, ICLR 2023 &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
POET (Ours) & 87.9 & \cellcolor{magenta!20}84.9 & \cellcolor{yellow!30}65.6 & 82.8 & \cellcolor{magenta!20}80.3 & \cellcolor{yellow!30}45.8 & 76.8 & \cellcolor{magenta!20}69.5 & \cellcolor{yellow!30}60.0 & 68.6 & \cellcolor{magenta!20}59.3 & \cellcolor{yellow!30}\textbf{57.4} & \cellcolor{gray!20}\textbf{59.2} & 
\textcolor{red}{\textbf{58.3}} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{sota activity}
% \vspace{-0.2in}
\end{table*}

\vspace{-0.2in}
\begin{table*}[h]
% \tiny
\setlength{\tabcolsep}{3pt}
\centering
\caption{Performance on SHREC-2017 \cite{10.2312:3dor.20171049} \textbf{Gesture Recognition benchmark}, based on DG-STA \cite{chen2019construct} graph transformer backbone. Reporting mean and STD across 5 runs.}
\label{SOTA gesture}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}llllllllllll@{}} \toprule 
& \task{0} 
& \multicolumn{3}{c}{\task{1}} 
& \multicolumn{3}{c}{\task{2}} 
& \multicolumn{4}{c}{\task{3}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(l){9-12} 
Method & Base & Old & New & Avg & Old & New & Avg & Old & New & \textbf{Avg} & $\boldsymbol A_{HM}$  \\
\hline
Joint (Oracle) & 88.8 & 91.2 $\pm$ 0.4 & 37.5 $\pm$ 3.0 & 79.4 $\pm$ 0.7 & 91.4 $\pm$ 1.1 & 52.2 $\pm$ 4.2 & 77.3 $\pm$ 2.1 & \cellcolor{magenta!20}\textbf{90.8 $\pm$ 0.2} & \cellcolor{yellow!30}47.6 $\pm$ 2.8 & \cellcolor{gray!20}\textbf{70.9 $\pm$ 1.2} & \textcolor{red}{\textbf{62.4 $\pm$ 0.4}} \\
\hline
FT & 88.8 & \phantom{0}0.0 & 91.6 $\pm$ 3.7 & 20.3 $\pm$ 0.8 & \phantom{0}0.0 & 69.5 $\pm$ 11.9 & 12.4 $\pm$ 2.1 & \cellcolor{magenta!20}\phantom{0}0.0 & \cellcolor{yellow!30}85.8 $\pm$ 9.4 & 13.4 $\pm$ 1.5 & \phantom{0}0.0 \\
FE & 88.8 & 56.2 $\pm$ 3.4 & 85.7 $\pm$ 6.5 & 62.7 $\pm$ 2.4 & 37.2 $\pm$ 6.7 & 64.3 $\pm$ 11.9 & 41.9 $\pm$ 6.9 & \cellcolor{magenta!20}17.5 $\pm$ 5.1 & \cellcolor{yellow!30}77.3 $\pm$ 8.8 & 26.8 $\pm$ 3.4 & 28.5 $\pm$ 6.4 \\
FE, frozen & 88.8 & 69.6 $\pm$ 4.1 & 77.4 $\pm$ 9.2 & 71.3 $\pm$ 1.9 & 61.9 $\pm$ 2.1 & 59.1 $\pm$ 11.7 & 61.4 $\pm$ 2.7 & \cellcolor{magenta!20}44.7 $\pm$ 3.2 & 54.5 $\pm$ 6.7 & 46.2 $\pm$ 2.7 & 49.1 $\pm$ 4.3 \\
LWF \cite{li2017learning} & 88.8 & \phantom{0}0.0 & 91.2 $\pm$ 6.2 & 20.2 $\pm$ 1.4 & \phantom{0}0.0 & 70.3 $\pm$ 5.8 & 12.5 $\pm$ 1.0 & \phantom{0}0.0 & \textbf{88.4 $\pm$ 13.7} & 13.8 $\pm$ 2.1 & \phantom{0}0.0 \\
L2P \cite{wang2022learning} & 88.8 & 17.3 $\pm$ 5.2 & 30.9 $\pm$ 25.9 & 20.3 $\pm$ 5.9 & 12.3 $\pm$ 5.9 & \phantom{0}2.1 $\pm$ 3.8 & 10.5 $\pm$ 4.8 & \phantom{0}8.2 $\pm$ 4.0 & \phantom{0}6.9 $\pm$ 8.5 & \phantom{0}7.9 $\pm$ 3.9 & \phantom{0}7.5 $\pm$ 5.5 \\
CODA-P \cite{smith2023coda}** & 87.7 & 19.9 $\pm$ 5.6 & \phantom{0}0.5 $\pm$ 0.7 & 15.6 $\pm$ 4.5 & 13.6 $\pm$ 4.0 & \phantom{0}2.2 $\pm$ 1.9 & 11.6 $\pm$ 1.9 & \phantom{0}7.9 $\pm$ 1.8 & 14.1 $\pm$ 21.4 & \phantom{0}8.8 $\pm$ 2.4 & 10.1 $\pm$ 3.2 \\
ALICE \cite{peng2022few} & 92.1 & 86.0 $\pm$ 3.5 & 24.5 $\pm$ 14.9 & 72.4 $\pm$ 5.7 & 72.1 $\pm$ 5.7 & 22.5 $\pm$ 16.9 & 63.3 $\pm$ 7.6 & \cellcolor{magenta!20}\textbf{62.5 $\pm$ 6.8} & \cellcolor{yellow!30}11.9 $\pm$ 9.9 & \cellcolor{gray!20}\textbf{54.6} $\pm$ 6.9 & 20.0 $\pm$ 8.1 \\
\hline
POET (Ours) & 91.9  & 71.1 $\pm$ 4.7 & 80.8 $\pm$ 6.7 & 73.2 $\pm$ 3.7 & 63.1 $\pm$ 2.2 & 56.7 $\pm$ 9.4 & 61.9 $\pm$ 1.8 & \cellcolor{magenta!20}45.9 $\pm$ 2.6 & \cellcolor{yellow!30}72.4 $\pm$ 7.1 & \cellcolor{gray!20}50.0 $\pm$ 1.6 & \textcolor{red}{\textbf{56.2 $\pm$ 1.6}} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-0.2in}
\end{table*}




==> Sections/test.tex <==
\begin{table*}[t]
% \tiny
\setlength{\tabcolsep}{3pt}
\centering
\caption{\scriptsize \textbf{Gesture Recognition Results (\%, $\uparrow$), Comparison with SOTA:} SHREC 2017 \cite{10.2312:3dor.20171049} dataset on DG-STA \cite{chen2019construct} graph transformer backbone. Reporting mean and standard deviation across 5 runs. Bracket accuracy difference is wrt POET. \textbf{POET achieves best $A_{HM}=56.2\%$}.}
\label{SOTA gesture}
\vspace{-6pt}
\begin{adjustbox}{width=0.90\textwidth}
\begin{tabular}{@{}llHHlHHlllll@{}} \toprule 
& $\mathcal{UB}^{(0)}$
& \multicolumn{3}{c}{\task{1}} 
& \multicolumn{3}{c}{\task{2}} 
& \multicolumn{4}{c}{\task{3}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(l){9-12} 
Method & Base & Old & New & Avg & Old & New & Avg & Old & New & Avg & $A_{HM}$  \\
\hline
\cellcolor{orange!15}Joint (Oracle) & 88.8 & 91.2 $\pm$ 0.4 & 37.5 $\pm$ 3.0 & 79.4 $\pm$ 0.7 & 91.4 $\pm$ 1.1 & 52.2 $\pm$ 4.2 & 77.3 $\pm$ 2.1 &  &  & \cellcolor{gray!20}\textbf{70.9 $\pm$ 1.2} & \textcolor{red}{\textbf{62.4 $\pm$ 0.4}} \\
% Joint (Oracle) & 88.8 & 91.2 $\pm$ 0.4 & 37.5 $\pm$ 3.0 & 79.4 $\pm$ 0.7 & 91.4 $\pm$ 1.1 & 52.2 $\pm$ 4.2 & 77.3 $\pm$ 2.1 & \cellcolor{white!20}\textbf{90.8 $\pm$ 0.2} & \cellcolor{white!30}47.6 $\pm$ 2.8 & \cellcolor{gray!20}\textbf{70.9 $\pm$ 1.2} & \textcolor{red}{\textbf{62.4 $\pm$ 0.4}} \\
\hline
FT & 88.8 & \phantom{0}0.0 & 91.6 $\pm$ 3.7 & 20.3 $\pm$ 0.8 & \phantom{0}0.0 & 69.5 $\pm$ 11.9 & 12.4 $\pm$ 2.1 & \cellcolor{white!20}\phantom{0}0.0 & \cellcolor{white!30}85.8 $\pm$ 9.4 & 13.4 $\pm$ 1.5 & \phantom{0}0.0 \\
FE & 88.8 & 56.2 $\pm$ 3.4 & 85.7 $\pm$ 6.5 & 62.7 $\pm$ 2.4 & 37.2 $\pm$ 6.7 & 64.3 $\pm$ 11.9 & 41.9 $\pm$ 6.9 & \cellcolor{white!20}17.5 $\pm$ 5.1 & \cellcolor{white!30}77.3 $\pm$ 8.8 & 26.8 $\pm$ 3.4 & 28.5 $\pm$ 6.4 \\
\cellcolor{gray!15}FE, Frozen & \cellcolor{gray!15}88.8 & 69.6 $\pm$ 4.1 & 77.4 $\pm$ 9.2 & \cellcolor{gray!15}71.3 $\pm$ 1.9 & \cellcolor{gray!15}61.9 $\pm$ 2.1 & 59.1 $\pm$ 11.7 & \cellcolor{gray!15}61.4 $\pm$ 2.7 & \cellcolor{gray!15}44.7 $\pm$ 3.2 \textcolor{red}{(-1.2)} & \cellcolor{gray!15}54.5 $\pm$ 6.7 \textcolor{red}{(-17.9)} & \cellcolor{gray!15}46.2 $\pm$ 2.7 & \cellcolor{gray!15}49.1 $\pm$ 4.3 \\
LWF \cite{li2017learning} & 88.8 & \phantom{0}0.0 & 91.2 $\pm$ 6.2 & 20.2 $\pm$ 1.4 & \phantom{0}0.0 & 70.3 $\pm$ 5.8 & 12.5 $\pm$ 1.0 & \phantom{0}0.0 & \textbf{88.4 $\pm$ 13.7} & 13.8 $\pm$ 2.1 & \phantom{0}0.0 \\
L2P \cite{wang2022learning} & 88.8 & 17.3 $\pm$ 5.2 & 30.9 $\pm$ 25.9 & 20.3 $\pm$ 5.9 & 12.3 $\pm$ 5.9 & \phantom{0}2.1 $\pm$ 3.8 & 10.5 $\pm$ 4.8 & \phantom{0}8.2 $\pm$ 4.0 & \phantom{0}6.9 $\pm$ 8.5 & \phantom{0}7.9 $\pm$ 3.9 & \phantom{0}7.5 $\pm$ 5.5 \\
CODA-P \cite{smith2023coda}** & 87.7 & 19.9 $\pm$ 5.6 & \phantom{0}0.5 $\pm$ 0.7 & 15.6 $\pm$ 4.5 & 13.6 $\pm$ 4.0 & \phantom{0}2.2 $\pm$ 1.9 & 11.6 $\pm$ 1.9 & \phantom{0}7.9 $\pm$ 1.8 & 14.1 $\pm$ 21.4 & \phantom{0}8.8 $\pm$ 2.4 & 10.1 $\pm$ 3.2 \\
\cellcolor{gray!15}ALICE \cite{peng2022few} & \cellcolor{gray!15}92.1 & 86.0 $\pm$ 3.5 & 24.5 $\pm$ 14.9 & \cellcolor{gray!15}72.4 $\pm$ 5.7 & 72.1 $\pm$ 5.7 & 22.5 $\pm$ 16.9 & \cellcolor{gray!15}63.3 $\pm$ 7.6 & \cellcolor{gray!15}\textbf{62.5 $\pm$ 6.8} \textcolor{blue}{(+16.6)} & \cellcolor{gray!15}11.9 $\pm$ 9.9 \textcolor{red}{(-60.5)} & \cellcolor{gray!15}\textbf{54.6} $\pm$ 6.9 & \cellcolor{gray!15}20.0 $\pm$ 8.1 \textcolor{red}{(-36.2)} \\
\hline
\cellcolor{gray!20}POET (Ours) & \cellcolor{gray!20}91.9  & 71.1 $\pm$ 4.7 & 80.8 $\pm$ 6.7 & \cellcolor{gray!20}73.2 $\pm$ 3.7 & 63.1 $\pm$ 2.2 & 56.7 $\pm$ 9.4 & \cellcolor{gray!20}61.9 $\pm$ 1.8 & \cellcolor{gray!20}45.9 $\pm$ 2.6 & \cellcolor{gray!20}72.4 $\pm$ 7.1 & \cellcolor{gray!20}50.0 $\pm$ 1.6 & \cellcolor{gray!20}\textcolor{red}{\textbf{56.2 $\pm$ 1.6}} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}
\end{table*} 

==> Tables/main-table-v2.tex <==


\begin{table*}[t]
% \scriptsize
\setlength{\tabcolsep}{5pt}
\centering
\caption{\scriptsize \textbf{Activity Recognition Results (\%, $\uparrow$), Comparison with SOTA:}
}
\vspace{-6pt}
\begin{adjustbox}{width=0.98\textwidth}
\begin{tabular}{@{}llHHlHHlHHlllll@{}} \toprule 
& \normalsize $\boldsymbol{\mathcal{UB}^{(0)}}$
& \multicolumn{3}{c}{\normalsize \tabletask{1}} 
& \multicolumn{3}{c}{\normalsize \tabletask{2}}
& \multicolumn{3}{c}{\normalsize \tabletask{3}}
& \multicolumn{4}{c}{\normalsize \tabletask{4}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}  \cmidrule(l){12-15} 
Method & Average Acc & Old & New & Average Acc & Old & New & Average Acc & Old & New & Average Acc & Old & New & Average Acc & $A_{HM}$  \\
% \textbf{Method} & \textbf{Base} & \textbf{Old} & \textbf{New} & \textbf{Average Acc} & \textbf{Old} & \textbf{New} & \textbf{Average Acc} & \textbf{Old} & \textbf{New} & \textbf{Average Acc} & \textbf{Old} & \textbf{New} & \textbf{Average Acc} & \textbf{$\boldsymbol{A_{HM}}$}  \\
\hline
\hline
\cellcolor{orange!15}Joint (Oracle)  & 88.4 &  &  & 79.0 &  &  & 71.0 &  &  & 66.8 &  &  & \cellcolor{gray!20}\textbf{63.5}  \textcolor{white}{(+4.3)} &  \\
\cellcolor{orange!15}Joint POET (Oracle) &  & \multicolumn{3}{l}{} &  &  &  &  &  &  &  &  & \cellcolor{gray!20}\textcolor{black}{\textbf{67.2}}  \textcolor{white}{(+8.0)} &  \\
% \cellcolor{orange!15}FE, Task-Specific\^ & 88.4 & \cellcolor{white!20}76.5 & \cellcolor{white!30}59.1 & 59.1\^ & \cellcolor{white!20}77.8 & \cellcolor{white!30}39.4 & 39.4\^ & \cellcolor{white!20}76.0 & \cellcolor{white!30}45.5 & 45.5\^ & \cellcolor{white!20}\textbf{72.1}  \textcolor{white}{(+12.8)} & \cellcolor{white!30}38.8  \textcolor{white}{(-18.6)} & NA & NA \\
% \cellcolor{orange!15}FE$+$Replay & 88.4 &  &  & 81.0 &  &  & 74.9 &  &  & 71.9 & 29.7  \textcolor{white}{(-29.6)} & 72.8  \textcolor{white}{(+15.4)} & 69.2  \textcolor{white}{(+10.0)} & 42.2  \textcolor{white}{(-16.1)}  \\
% Task-Specific\^ &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
\cellcolor{gray!15}FE & \cellcolor{gray!15}88.4 &  &  & \cellcolor{gray!15}72.0 $\pm$ \scriptsize 1.1 &  &  & \cellcolor{gray!15}60.4 $\pm$ \scriptsize 2.4 &  &  & \cellcolor{gray!15}47.7 $\pm$ \scriptsize 2.1 & \cellcolor{gray!15}40.0 $\pm$ \scriptsize 1.6  \textcolor{white}{()} & \cellcolor{gray!15}51.0 $\pm$ \scriptsize 2.3  \textcolor{white}{()} & \cellcolor{gray!15}40.9 $\pm$ \scriptsize 1.4 & \cellcolor{gray!15}44.8 $\pm$ \scriptsize 1.1  \textcolor{white}{()} \\
FE, Frozen & 88.4 &  &  & 76.1 $\pm$ \scriptsize 1.0 &  &  & 52.4 $\pm$ \scriptsize 4.1 &  &  & 38.3 $\pm$ \scriptsize 2.7 & \cellcolor{white!20}28.4 $\pm$ \scriptsize 1.6 & \cellcolor{white!30}22.4 $\pm$ \scriptsize 4.5 & 27.9 $\pm$ \scriptsize 1.4 & 24.8 $\pm$ \scriptsize 3.0 \\
% FE$+$Replay$\dagger$ & 88.4 & 73.5 & 70.1 & 73.1 & 59.2 & 71.0 & 60.4 & 61.8 & 59.4 & 61.6 & 60.3 & 28.8 & 57.7 & 39.0 \\
FT & 88.4 & \phantom{0} &  & \phantom{0}6.2 $\pm$ \scriptsize 1.4 & \phantom{0} &  & \phantom{0}4.3 $\pm$ \scriptsize 1.5 & \phantom{0} &  & \phantom{0}2.8 $\pm$ \scriptsize 1.0 & \cellcolor{white!20}\phantom{0}0.2 $\pm$ \scriptsize 0.5 & \cellcolor{white!30}36.0 $\pm$ \scriptsize 10.1 & \phantom{0}3.2 $\pm$ \scriptsize 0.8 & \phantom{0}0.3 $\pm$ \scriptsize 1.0 \\

\hline
% LWF \cite{li2017learning} & 88.4 & \phantom{0}0.5 & 74.0 & \phantom{0}8.7 & \phantom{0}0.0 & 31.5 & \phantom{0}3.2 & \phantom{0}0.0 & 31.4 & \phantom{0}2.9 & \phantom{0}0.0  \textcolor{white}{(-59.3)} & 23.1 & \phantom{0}1.9 & \phantom{0}0.0 \\
EWC \cite{kirkpatrick2017overcoming} & 88.4 & \phantom{0} & & \phantom{0}6.6 $\pm$ \scriptsize 1.5 & \phantom{0} &  & \phantom{0}4.1 $\pm$ \scriptsize 1.4 & \phantom{0} &  & \phantom{0}3.1 $\pm$ \scriptsize 0.9 & \phantom{0}0.0 $\pm$ \scriptsize 0.0  \textcolor{white}{()} & 42.1 $\pm$ \scriptsize 9.5 & \phantom{0}3.5 $\pm$ \scriptsize 0.8 & \phantom{0}0.0 $\pm$ \scriptsize 0.0 \\
% Experience Replay & 88.4 &  &  & 34.1 &  &  & 46.4 &  &  & 46.3 & 50.3  \textcolor{white}{(-9.0)} & 25.4 & 48.3 & 33.8 \\
% Experience Replay$\dagger$ & 88.4 & \phantom{0}0.4 & 59.8 & \phantom{0}7.0 & \phantom{0}6.1 & \phantom{0}5.2 & \phantom{0}6.0 & \phantom{0}6.8 & 42.2 & 10.0 & 10.1 & 32.2 & 12.0 & 15.4 \\
LUCIR \cite{hou2019learning} & 87.9 & \phantom{0}0.0 &  & \phantom{0}4.3 $\pm$ \scriptsize 2.1 & \phantom{0}0.0 &  & \phantom{0}4.1 $\pm$ \scriptsize 1.3 & \phantom{0}0.0 & & \phantom{0}2.7 $\pm$ \scriptsize 0.8 & \phantom{0}0.2 $\pm$ \scriptsize 0.4  \textcolor{white}{()} & 26.0 $\pm$ \scriptsize 9.2 & \phantom{0}2.3 $\pm$ \scriptsize 0.9 & \phantom{0}0.4 $\pm$ \scriptsize 0.8 \\

\hline
% \cellcolor{gray!15}CODA-P \cite{smith2023coda}* & \cellcolor{gray!15}87.4 & 86.1 & \phantom{0}4.0 & \cellcolor{gray!15}76.3 & 76.0 & \phantom{0}0.3 & \cellcolor{gray!15}68.4 & 65.9 & \phantom{0}0.2 & \cellcolor{gray!15}59.7 & \cellcolor{gray!15}60.9  \textcolor{white}{(+1.6)} & \cellcolor{gray!15}\phantom{0}0.7  \textcolor{white}{(-56.7)} & \cellcolor{gray!15}55.7  \textcolor{white}{(-3.5)} & \cellcolor{gray!15}\phantom{0}1.3  \\
% CODA-P \cite{smith2023coda}** & 87.6 & \phantom{0}4.9 & \phantom{0}7.4 & \phantom{0}4.5 & 31.7 & \phantom{0}0.0 & 28.8 & \phantom{0}0.5 & \phantom{0}1.6 & \phantom{0}0.6 & 35.4 & \phantom{0}0.7 & 31.1 & \phantom{0}1.3 \\
% \cellcolor{gray!15}L2P \cite{wang2022learning}* & \cellcolor{gray!15}\textbf{88.6} & 88.4 & \phantom{0}0.0 & \cellcolor{gray!15}78.5  & 78.5 & \phantom{0}0.0 & \cellcolor{gray!15}70.7 & 70.1 & \phantom{0}0.0 & \cellcolor{gray!15}63.7 & \cellcolor{gray!15}61.2  \textcolor{white}{(+1.9)} & \cellcolor{gray!15}\phantom{0}0.0  \textcolor{white}{(-57.4)} & \cellcolor{gray!15}56.2  \textcolor{white}{(-3.0)} & \cellcolor{gray!15}\phantom{0}0.0  \\
% L2P \cite{wang2022learning}**  & 84.7 & \phantom{0}3.0 & \phantom{0}0.4 & \phantom{0}2.7 & \phantom{0}3.1 & \phantom{0}0.0 & \phantom{0}2.8 & \phantom{0}2.8 & \phantom{0}0.0 & \phantom{0}2.6 & \phantom{0}2.4 & \phantom{0}0.4 & \phantom{0}2.2 & \phantom{0}0.6 \\
% APT \cite{bowman2023carte}\^ & 86.6 & \phantom{0}NA & 29.2 & 29.2\^ & \phantom{0}NA & 30.6 & 30.6\^ & \phantom{0}NA & 35.9 & 35.9\^ & \phantom{0}NA & 35.0  \textcolor{white}{(-22.4)} & \phantom{0}NA & \phantom{0}NA \\
% ALICE \cite{peng2022few} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% NC-FSCIL, ICLR 2023 &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
\cellcolor{gray!20}POET (Ours) & \cellcolor{gray!20}87.9 & \cellcolor{gray!20} & \cellcolor{white!30} & \cellcolor{gray!20}\textbf{82.3 $\pm$ \scriptsize 0.6} & \cellcolor{white!20} & \cellcolor{white!30} & \cellcolor{gray!20}\textbf{76.8 $\pm$ \scriptsize 0.9} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}\textbf{68.4 $\pm$ \scriptsize 0.7} & \cellcolor{gray!20}57.2 $\pm$ \scriptsize 1.0 & \cellcolor{gray!20}\textbf{55.8 $\pm$ \scriptsize 5.9} & \cellcolor{gray!20}\textbf{57.1 $\pm$ \scriptsize 1.1} & 
\cellcolor{gray!20}\textbf{56.3 $\pm$ \scriptsize 3.2} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{sota activity}
\vspace{-10pt}
\end{table*}

==> Tables/main_table_diff_old.tex <==
% main table with diffrence markers intact 

\begin{table*}[t]
% \scriptsize
\setlength{\tabcolsep}{4pt}
\centering
\caption{\scriptsize \textbf{Activity Recognition Results (\%, $\uparrow$), Comparison with SOTA:}
}
\vspace{-6pt}
\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{@{}llHHlHHlHHlllll@{}} \toprule 
& $\mathcal{UB}^{(0)}$
& \multicolumn{3}{c}{\task{1}} 
& \multicolumn{3}{c}{\task{2}} 
& \multicolumn{3}{c}{\task{3}} 
& \multicolumn{4}{c}{\task{4}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}  \cmidrule(l){12-15} 
Method & Base & Old & New & Avg & Old & New & Avg & Old & New & Avg & Old & New & Avg & $A_{HM}$  \\
\hline
\cellcolor{orange!15}Joint (Oracle)  & 88.4 &  &  & 79.0 &  &  & 71.0 &  &  & 66.8 &  &  & \cellcolor{gray!20}\textbf{63.5} \textcolor{blue}{(+4.3)} &  \\
\cellcolor{orange!15}Joint POET (Oracle) &  & \multicolumn{3}{l}{} &  &  &  &  &  &  &  &  & \cellcolor{gray!20}\textcolor{black}{\textbf{67.2}} \textcolor{blue}{(+8.0)} &  \\
% \cellcolor{orange!15}FE, Task-Specific\^ & 88.4 & \cellcolor{white!20}76.5 & \cellcolor{white!30}59.1 & 59.1\^ & \cellcolor{white!20}77.8 & \cellcolor{white!30}39.4 & 39.4\^ & \cellcolor{white!20}76.0 & \cellcolor{white!30}45.5 & 45.5\^ & \cellcolor{white!20}\textbf{72.1} \textcolor{blue}{(+12.8)} & \cellcolor{white!30}38.8 \textcolor{red}{(-18.6)} & NA & NA \\
% \cellcolor{orange!15}FE$+$Replay & 88.4 &  &  & 81.0 &  &  & 74.9 &  &  & 71.9 & 29.7 \textcolor{red}{(-29.6)} & 72.8 \textcolor{blue}{(+15.4)} & 69.2 \textcolor{blue}{(+10.0)} & 42.2 \textcolor{red}{(-16.1)}  \\
% Task-Specific\^ &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
\cellcolor{gray!15}FE & \cellcolor{gray!15}88.4 &  &  & \cellcolor{gray!15}72.0 $\pm$ \scriptsize 1.1 &  &  & \cellcolor{gray!15}60.4 $\pm$ \scriptsize 2.4 &  &  & \cellcolor{gray!15}47.7 $\pm$ \scriptsize 2.1 & \cellcolor{gray!15}40.0 $\pm$ \scriptsize 1.6 \textcolor{red}{()} & \cellcolor{gray!15}51.0 $\pm$ \scriptsize 2.3 \textcolor{red}{()} & \cellcolor{gray!15}40.9 $\pm$ \scriptsize 1.4 & \cellcolor{gray!15}44.8 $\pm$ \scriptsize 1.1 \textcolor{red}{()} \\
FE, Frozen & 88.4 &  &  & 76.1 $\pm$ \scriptsize 1.0 &  &  & 52.4 $\pm$ \scriptsize 4.1 &  &  & 38.3 $\pm$ \scriptsize 2.7 & \cellcolor{white!20}28.4 $\pm$ \scriptsize 1.6 & \cellcolor{white!30}22.4 $\pm$ \scriptsize 4.5 & 27.9 $\pm$ \scriptsize 1.4 & 24.8 $\pm$ \scriptsize 3.0 \\
% FE$+$Replay$\dagger$ & 88.4 & 73.5 & 70.1 & 73.1 & 59.2 & 71.0 & 60.4 & 61.8 & 59.4 & 61.6 & 60.3 & 28.8 & 57.7 & 39.0 \\
FT & 88.4 & \phantom{0} &  & \phantom{0}6.2 $\pm$ \scriptsize 1.4 & \phantom{0} &  & \phantom{0}4.3 $\pm$ \scriptsize 1.5 & \phantom{0} &  & \phantom{0}2.8 $\pm$ \scriptsize 1.0 & \cellcolor{white!20}\phantom{0}0.2 $\pm$ \scriptsize 0.5 & \cellcolor{white!30}36.0 $\pm$ \scriptsize 10.1 & \phantom{0}3.2 $\pm$ \scriptsize 0.8 & \phantom{0}0.3 $\pm$ \scriptsize 1.0 \\

\hline
% LWF \cite{li2017learning} & 88.4 & \phantom{0}0.5 & 74.0 & \phantom{0}8.7 & \phantom{0}0.0 & 31.5 & \phantom{0}3.2 & \phantom{0}0.0 & 31.4 & \phantom{0}2.9 & \phantom{0}0.0 \textcolor{red}{(-59.3)} & 23.1 & \phantom{0}1.9 & \phantom{0}0.0 \\
EWC \cite{kirkpatrick2017overcoming} & 88.4 & \phantom{0} & & \phantom{0}6.6 $\pm$ \scriptsize 1.5 & \phantom{0} &  & \phantom{0}4.1 $\pm$ \scriptsize 1.4 & \phantom{0} &  & \phantom{0}3.1 $\pm$ \scriptsize 0.9 & \phantom{0}0.0 $\pm$ \scriptsize 0.0 \textcolor{red}{()} & 42.1 $\pm$ \scriptsize 9.5 & \phantom{0}3.5 $\pm$ \scriptsize 0.8 & \phantom{0}0.0 $\pm$ \scriptsize 0.0 \\
% Experience Replay & 88.4 &  &  & 34.1 &  &  & 46.4 &  &  & 46.3 & 50.3 \textcolor{red}{(-9.0)} & 25.4 & 48.3 & 33.8 \\
% Experience Replay$\dagger$ & 88.4 & \phantom{0}0.4 & 59.8 & \phantom{0}7.0 & \phantom{0}6.1 & \phantom{0}5.2 & \phantom{0}6.0 & \phantom{0}6.8 & 42.2 & 10.0 & 10.1 & 32.2 & 12.0 & 15.4 \\
LUCIR \cite{hou2019learning} & 87.9 & \phantom{0}0.0 &  & \phantom{0}4.3 $\pm$ \scriptsize 2.1 & \phantom{0}0.0 &  & \phantom{0}4.1 $\pm$ \scriptsize 1.3 & \phantom{0}0.0 & & \phantom{0}2.7 $\pm$ \scriptsize 0.8 & \phantom{0}0.2 $\pm$ \scriptsize 0.4 \textcolor{red}{()} & 26.0 $\pm$ \scriptsize 9.2 & \phantom{0}2.3 $\pm$ \scriptsize 0.9 & \phantom{0}0.4 $\pm$ \scriptsize 0.8 \\

\hline
% \cellcolor{gray!15}CODA-P \cite{smith2023coda}* & \cellcolor{gray!15}87.4 & 86.1 & \phantom{0}4.0 & \cellcolor{gray!15}76.3 & 76.0 & \phantom{0}0.3 & \cellcolor{gray!15}68.4 & 65.9 & \phantom{0}0.2 & \cellcolor{gray!15}59.7 & \cellcolor{gray!15}60.9 \textcolor{blue}{(+1.6)} & \cellcolor{gray!15}\phantom{0}0.7 \textcolor{red}{(-56.7)} & \cellcolor{gray!15}55.7 \textcolor{red}{(-3.5)} & \cellcolor{gray!15}\phantom{0}1.3  \\
% CODA-P \cite{smith2023coda}** & 87.6 & \phantom{0}4.9 & \phantom{0}7.4 & \phantom{0}4.5 & 31.7 & \phantom{0}0.0 & 28.8 & \phantom{0}0.5 & \phantom{0}1.6 & \phantom{0}0.6 & 35.4 & \phantom{0}0.7 & 31.1 & \phantom{0}1.3 \\
% \cellcolor{gray!15}L2P \cite{wang2022learning}* & \cellcolor{gray!15}\textbf{88.6} & 88.4 & \phantom{0}0.0 & \cellcolor{gray!15}78.5  & 78.5 & \phantom{0}0.0 & \cellcolor{gray!15}70.7 & 70.1 & \phantom{0}0.0 & \cellcolor{gray!15}63.7 & \cellcolor{gray!15}61.2 \textcolor{blue}{(+1.9)} & \cellcolor{gray!15}\phantom{0}0.0 \textcolor{red}{(-57.4)} & \cellcolor{gray!15}56.2 \textcolor{red}{(-3.0)} & \cellcolor{gray!15}\phantom{0}0.0  \\
% L2P \cite{wang2022learning}**  & 84.7 & \phantom{0}3.0 & \phantom{0}0.4 & \phantom{0}2.7 & \phantom{0}3.1 & \phantom{0}0.0 & \phantom{0}2.8 & \phantom{0}2.8 & \phantom{0}0.0 & \phantom{0}2.6 & \phantom{0}2.4 & \phantom{0}0.4 & \phantom{0}2.2 & \phantom{0}0.6 \\
% APT \cite{bowman2023carte}\^ & 86.6 & \phantom{0}NA & 29.2 & 29.2\^ & \phantom{0}NA & 30.6 & 30.6\^ & \phantom{0}NA & 35.9 & 35.9\^ & \phantom{0}NA & 35.0 \textcolor{red}{(-22.4)} & \phantom{0}NA & \phantom{0}NA \\
% ALICE \cite{peng2022few} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% NC-FSCIL, ICLR 2023 &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
\cellcolor{gray!20}POET (Ours) & \cellcolor{gray!20}87.9 & \cellcolor{gray!20} & \cellcolor{white!30} & \cellcolor{gray!20}\textbf{82.3 $\pm$ \scriptsize 0.6} & \cellcolor{white!20} & \cellcolor{white!30} & \cellcolor{gray!20}\textbf{76.8 $\pm$ \scriptsize 0.9} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}\textbf{68.4 $\pm$ \scriptsize 0.7} & \cellcolor{gray!20}57.2 $\pm$ \scriptsize 1.0 & \cellcolor{gray!20}\textbf{55.8 $\pm$ \scriptsize 5.9} & \cellcolor{gray!20}\textbf{57.1 $\pm$ \scriptsize 1.1} & 
\cellcolor{gray!20}\textcolor{red}{\textbf{56.3 $\pm$ \scriptsize 3.2}} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{sota activity}
\vspace{-10pt}
\end{table*}




% \vspace{-6pt}
% \begin{table*}[h]
% % \scriptsize
% \setlength{\tabcolsep}{4pt}
% \centering
% \caption{\scriptsize \textbf{Activity Recognition Results (\%, $\uparrow$), Comparison with SOTA:} NTU RGB+D \cite{shahroudy2016ntu} dataset on CTR-GCN \cite{chen2021channel} backbone. After training on each incremental task, we report Average of all classes seen so far (`Avg'). We also report (i) $A_{HM}$, (ii) only old classes accuracy (`Old'), (iii) only new classes accuracy (`New') in the last session. Numbers in brackets are wrt POET. \textit{POET achieves the best stability-plasticity trade-off across all baselines indicated by the $A_{HM}=58.3\%$. POET also has the highest Avg across all user sessions outside of upper bound baselines \textcolor{orange}{in orange}.}
% % \textbf{Notation:} \textbf{\^} denotes standalone models trained and deployed for each task $T_i$ individually (note `Avg' is NA for these and `Old' refers to only base session \% for these); \textbf{$\dagger$} refers to storage and replay of all incremental session training data; \textbf{*} refers to concatenation of prompts along temporal dimension of input embedding $x_e$; and \textbf{**} concatenates along a rolled-out spatio-temporal dimension of $x_e$.
% }
% \vspace{-6pt}
% \begin{adjustbox}{width=0.8\textwidth}
% \begin{tabular}{@{}llHHlHHlHHlllll@{}} \toprule 
% & $\mathcal{UB}^{(0)}$
% & \multicolumn{3}{c}{\task{1}} 
% & \multicolumn{3}{c}{\task{2}} 
% & \multicolumn{3}{c}{\task{3}} 
% & \multicolumn{4}{c}{\task{4}} \\
% \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}  \cmidrule(l){12-15} 
% Method & Base & Old & New & Avg & Old & New & Avg & Old & New & Avg & Old & New & Avg & $A_{HM}$  \\
% \hline
% \cellcolor{orange!15}Joint (Oracle)  & 88.4 &  &  & 79.0 &  &  & 71.0 &  &  & 66.8 &  &  & \cellcolor{gray!20}\textbf{63.5} \textcolor{blue}{(+4.3)} &  \\
% \cellcolor{orange!15}Joint POET (Oracle) &  & \multicolumn{3}{l}{} &  &  &  &  &  &  &  &  & \cellcolor{gray!20}\textcolor{black}{\textbf{67.2}} \textcolor{blue}{(+8.0)} &  \\
% \cellcolor{orange!15}FE, Task-Specific\^ & 88.4 & \cellcolor{white!20}76.5 & \cellcolor{white!30}59.1 & 59.1\^ & \cellcolor{white!20}77.8 & \cellcolor{white!30}39.4 & 39.4\^ & \cellcolor{white!20}76.0 & \cellcolor{white!30}45.5 & 45.5\^ & \cellcolor{white!20}\textbf{72.1} \textcolor{blue}{(+12.8)} & \cellcolor{white!30}38.8 \textcolor{red}{(-18.6)} & NA & NA \\
% \cellcolor{orange!15}FE$+$Replay & 88.4 &  &  & 81.0 &  &  & 74.9 &  &  & 71.9 & 29.7 \textcolor{red}{(-29.6)} & 72.8 \textcolor{blue}{(+15.4)} & 69.2 \textcolor{blue}{(+10.0)} & 42.2 \textcolor{red}{(-16.1)}  \\
% % Task-Specific\^ &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \hline
% \cellcolor{gray!15}FE & \cellcolor{gray!15}88.4 & 76.5 & 59.1 & \cellcolor{gray!15}74.5 & 67.9 & 51.4 & \cellcolor{gray!15}66.3 & 50.4 & 40.8 & \cellcolor{gray!15}49.5 & \cellcolor{gray!15}39.2 \textcolor{red}{(-20.1)} & \cellcolor{gray!15}46.8 \textcolor{red}{(-10.6)} & \cellcolor{gray!15}39.9 & \cellcolor{gray!15}42.7 \textcolor{red}{(-15.6)} \\
% FE, Frozen & 88.4 & 81.7 & 49.2 & 78.1 & 64.7 & 40.0 & 62.3 & 43.2 & 27.6 & 41.7 & \cellcolor{white!20}29.5 & \cellcolor{white!30}25.5 & 29.2 & 27.4 \\
% FE$+$Replay$\dagger$ & 88.4 & 73.5 & 70.1 & 73.1 & 59.2 & 71.0 & 60.4 & 61.8 & 59.4 & 61.6 & 60.3 & 28.8 & 57.7 & 39.0 \\
% FT & 88.4 & \phantom{0}0.4 & 58.2 & \phantom{0}6.8 & \phantom{0}0.0 & 59.2 & \phantom{0}6.0 & \phantom{0}0.0 & 41.6 & \phantom{0}3.8 & \cellcolor{white!20}\phantom{0}0.0 & \cellcolor{white!30}25.1 & \phantom{0}2.1 & \phantom{0}0.0 \\
% \hline
% LWF \cite{li2017learning} & 88.4 & \phantom{0}0.5 & 74.0 & \phantom{0}8.7 & \phantom{0}0.0 & 31.5 & \phantom{0}3.2 & \phantom{0}0.0 & 31.4 & \phantom{0}2.9 & \phantom{0}0.0 \textcolor{red}{(-59.3)} & 23.1 & \phantom{0}1.9 & \phantom{0}0.0 \\
% EWC \cite{kirkpatrick2017overcoming} & 88.4 & \phantom{0}0.0 & 57.4 & \phantom{0}6.4 & \phantom{0}0.0 & 62.2 & \phantom{0}6.2 & \phantom{0}0.0 & 33.9 & \phantom{0}3.1 & \phantom{0}0.0 \textcolor{red}{(-59.3)} & 28.9 & \phantom{0}2.4 & \phantom{0}0.0 \\
% Experience Replay & 88.4 &  &  & 34.1 &  &  & 46.4 &  &  & 46.3 & 50.3 \textcolor{red}{(-9.0)} & 25.4 & 48.3 & 33.8 \\
% Experience Replay$\dagger$ & 88.4 & \phantom{0}0.4 & 59.8 & \phantom{0}7.0 & \phantom{0}6.1 & \phantom{0}5.2 & \phantom{0}6.0 & \phantom{0}6.8 & 42.2 & 10.0 & 10.1 & 32.2 & 12.0 & 15.4 \\
% LUCIR \cite{hou2019learning} & 87.9 & \phantom{0}0.0 & 19.9 & \phantom{0}2.2 & \phantom{0}0.0 & 20.1 & \phantom{0}2.0 & \phantom{0}0.0 & 29.2 & \phantom{0}2.7 & \phantom{0}1.3 \textcolor{red}{(-58.0)} & \phantom{0}2.5 & \phantom{0}1.4 & \phantom{0}0.0 \\
%  % &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \hline
% \cellcolor{gray!15}CODA-P \cite{smith2023coda}* & \cellcolor{gray!15}87.4 & 86.1 & \phantom{0}4.0 & \cellcolor{gray!15}76.3 & 76.0 & \phantom{0}0.3 & \cellcolor{gray!15}68.4 & 65.9 & \phantom{0}0.2 & \cellcolor{gray!15}59.7 & \cellcolor{gray!15}60.9 \textcolor{blue}{(+1.6)} & \cellcolor{gray!15}\phantom{0}0.7 \textcolor{red}{(-56.7)} & \cellcolor{gray!15}55.7 \textcolor{red}{(-3.5)} & \cellcolor{gray!15}\phantom{0}1.3  \\
% CODA-P \cite{smith2023coda}** & 87.6 & \phantom{0}4.9 & \phantom{0}7.4 & \phantom{0}4.5 & 31.7 & \phantom{0}0.0 & 28.8 & \phantom{0}0.5 & \phantom{0}1.6 & \phantom{0}0.6 & 35.4 & \phantom{0}0.7 & 31.1 & \phantom{0}1.3 \\
% \cellcolor{gray!15}L2P \cite{wang2022learning}* & \cellcolor{gray!15}\textbf{88.6} & 88.4 & \phantom{0}0.0 & \cellcolor{gray!15}78.5  & 78.5 & \phantom{0}0.0 & \cellcolor{gray!15}70.7 & 70.1 & \phantom{0}0.0 & \cellcolor{gray!15}63.7 & \cellcolor{gray!15}61.2 \textcolor{blue}{(+1.9)} & \cellcolor{gray!15}\phantom{0}0.0 \textcolor{red}{(-57.4)} & \cellcolor{gray!15}56.2 \textcolor{red}{(-3.0)} & \cellcolor{gray!15}\phantom{0}0.0  \\
% L2P \cite{wang2022learning}**  & 84.7 & \phantom{0}3.0 & \phantom{0}0.4 & \phantom{0}2.7 & \phantom{0}3.1 & \phantom{0}0.0 & \phantom{0}2.8 & \phantom{0}2.8 & \phantom{0}0.0 & \phantom{0}2.6 & \phantom{0}2.4 & \phantom{0}0.4 & \phantom{0}2.2 & \phantom{0}0.6 \\
% APT \cite{bowman2023carte}\^ & 86.6 & \phantom{0}NA & 29.2 & 29.2\^ & \phantom{0}NA & 30.6 & 30.6\^ & \phantom{0}NA & 35.9 & 35.9\^ & \phantom{0}NA & 35.0 \textcolor{red}{(-22.4)} & \phantom{0}NA & \phantom{0}NA \\
% % ALICE \cite{peng2022few} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% % NC-FSCIL, ICLR 2023 &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \hline
% \cellcolor{gray!20}POET (Ours) & \cellcolor{gray!20}87.9 & \cellcolor{gray!20}84.9 & \cellcolor{white!30}65.6 & \cellcolor{gray!20}\textbf{82.8} & \cellcolor{white!20}80.3 & \cellcolor{white!30}45.8 & \cellcolor{gray!20}\textbf{76.8} & \cellcolor{gray!20}69.5 & \cellcolor{gray!20}60.0 & \cellcolor{gray!20}\textbf{68.6} & \cellcolor{gray!20}59.3 & \cellcolor{gray!20}\textbf{57.4} & \cellcolor{gray!20}\textbf{59.2} & 
% \cellcolor{gray!20}\textcolor{red}{\textbf{58.3}} \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{sota activity}
% \vspace{-10pt}
% \end{table*}
